Improving Model Accuracy for Imbalanced Image Classification Tasks by Adding a Final Batch Normalization Layer: An Empirical Study

Some real-world domains, such as Agriculture and Healthcare, comprise early-stage disease indications whose recording constitutes a rare event, and yet, whose precise detection at that stage is critical. In this type of highly imbalanced classification problems, which encompass complex features, deep learning (DL) is much needed because of its strong detection capabilities. At the same time, DL is observed in practice to favor majority over minority classes and consequently suffer from inaccurate detection of the targeted early-stage indications. To simulate such scenarios, we artificially generate skewness (99% vs. 1%) for certain plant types out of the PlantVillage dataset as a basis for classification of scarce visual cues through transfer learning. By randomly and unevenly picking healthy and unhealthy samples from certain plant types to form a training set, we consider a base experiment as fine-tuning ResNet34 and VGG19 architectures and then testing the model performance on a balanced dataset of healthy and unhealthy images. We empirically observe that the initial F1 test score jumps from 0.29 to 0.95 for the minority class upon adding a final Batch Normalization (BN) layer just before the output layer in VGG19. We demonstrate that utilizing an additional BN layer before the output layer in modern CNN architectures has a considerable impact in terms of minimizing the training time and testing error for minority classes in highly imbalanced data sets. Moreover, when the final BN is employed, minimizing the loss function may not be the best way to assure a high F1 test score for minority classes in such problems. That is, the network might perform better even if it is not confident enough while making a prediction; leading to another discussion about why softmax output is not a good uncertainty measure for DL models.

==> BroaderImpact.tex <==
\section{Broader Impact}\label{sec:broaderImpact}
%Despite tremendous advances in computer vision and object recognition algorithms in the past few years, their effectiveness remains strongly dependent upon the datasets' size and distribution, which are usually limited under real-world settings.
This work is mostly concerned with hard classification problems at early-stages of diseases (either crop or human diseases), which suffer from lack of data instances, and whose effective treatment would make a dramatic impact on Agriculture and Healthcare. As an example, we mention the renowned Potato Blight disease, which is responsible for dramatic crop losses annually. This is mainly because the visual cues are hardly detectable at early stages, while the highly infectious nature leads rapidly to devastation in a large scale. Solving entirely the early-detection challenge of Potato Blight has thus the potential for a global impact on food production.
%, with hardly distinguishable indications and rare recording when it comes to rare anomalies like crop diseases in agriculture or malignant tumors in the medical domain. 
%Our approach presents an efficient way out of this dilemma and has large potential for the corresponding applications in precision agriculture and diagnostics in healthcare, to mention the most important ones. 
Moreover and without need to elaborate, early detection of lethal human diseases, and particularly accurate identification of early-stage malignant tumors, would make a major impact on healthcare.
Those and additional potential diseases detection adhere to the United Nation's sustainable development goals on ``zero hunger'' and ``good health''.

Moreover, in our collaborations with private and public partners, DL of imbalanced classification tasks will be utilized towards multiple sustainable development goals.
%\vk{instead of mentioning a private company, can we make all these issue a common problem in industry?} 
Examples include ecosystem service assessment by measuring city green with LIDAR data, automated insulation defect detection with thermography data, assessments of installed solar capacity based on earth observation data, and nature reserve monitoring with remote sensing and deep learning. However, class imbalance poses an obstacle in each of these applications. 
One example of this is in the determination of the type of nature with remote sensing for ecosystem preservation purposes. Here, it is crucial that less frequent types of nature are assessed accurately, as these are also often the areas that are most valuable from an ecological perspective. The inherent imbalance in nature maps makes deep learning models susceptible to under-representation of these areas in the results. This requires case-by-case engineering, and limits an impactful application of deep learning in this domain. 
Similarly, this poses a problem in identification of solar installation by analyzing images of hundreds of thousands of rooftops: most of these rooftops do not contain solar installations. Training models on images of rooftops with deep learning either requires excluding most of the rooftops without panels from the training dataset, or leads to a training dataset with a large class imbalance.

%\vk{we can still enrich this section? we have no space limitation beyond this point}
\begin{comment}
This work has the following potential positive impact in  society:
%
\begin{itemize}[leftmargin=.5cm]
    \item Despite tremendous advances in computer vision and object recognition algorithms in the past few years, the effectiveness of these algorithms depends on the size of the data which is usually not available under real world settings when it comes to rare anomalies like crop diseases in agriculture or malignant tumors in the medical domain. Our approach presents an efficient way out of this dilemma and has large potential for the corresponding applications in precision agriculture and diagnostics in healthcare, to mention the most important ones. 
    These potential application domains are relevant to the United Nation's sustainable development goals on ``zero hunger'' and ``good health''.
    
    \item Our study shows that we can still achieve substantial improvement using a smaller number of anomaly samples in the train set just by changing the neural network architecture with no additional cost. 
\end{itemize}
\end{comment}



==> deleted/References_old.tex <==

\section*{References}

[1] Hawkins, D. M., 1980), Identification of outliers (Vol. 11). London: Chapman and Hall.

[2] Beggel, L., Pfeiffer, M. and Bischl, B., 2019, Robust anomaly detection in images using adversarial autoencoders. arXiv preprint arXiv:1901.06355.

[3] Hussain, Mahbub and Bird, Jordan and Faria, Diego, 2018, A Study on CNN Transfer Learning for Image Classification. 

[4] Shorten, C., Khoshgoftaar, T.M., 2019, A survey on Image Data Augmentation for Deep Learning. J Big Data 6, 60. https://doi.org/10.1186/s40537-019-0197-0

[5] Barz, B., and Denzler, J., 2020, Deep learning on small datasets without pre-training using cosine loss. In The IEEE Winter Conference on Applications of Computer Vision (pp. 1371-1380).

[6] Lake, B. M., Salakhutdinov, R., and Tenenbaum, J. B., 2015, Human-level concept learning through probabilistic program induction. Science, 350(6266), 1332-1338.

[7] https://www.crowdai.org/challenges/plantvillage-disease-classification-challenge

[8] Hughes, D., and Salathé, M., 2015, An open access repository of images on plant health to enable the development of mobile disease diagnostics. arXiv preprint arXiv:1511.08060.

[9] Mohanty, S. P., Hughes, D. P., and Salathé, M., 2016, Using deep learning for image-based plant disease detection. Frontiers in plant science, 7, 1419.

[10] He, K., Zhang, X., Ren, S., and Sun, J., 2016, Deep residual learning for image recognition. In Proceedings of the IEEE conference on computer vision and pattern recognition (pp. 770-778).

[11] Simonyan, K., and Zisserman, A., 2014, Very deep convolutional networks for large-scale image recognition. arXiv preprint arXiv:1409.1556.

[12] Gutman, D., Codella, N. C., Celebi, E., Helba, B., Marchetti, M., Mishra, N., and Halpern, A., 2016, Skin lesion analysis toward melanoma detection: A challenge at the international symposium on biomedical imaging (ISBI) 2016, hosted by the international skin imaging collaboration (ISIC). arXiv preprint arXiv:1605.01397.

[13] Zhang, L., Yang, F., Zhang, Y.D. and Zhu, Y.J., 2016, September. Road crack detection using deep convolutional neural network. In 2016 IEEE international conference on image processing (ICIP) (pp. 3708-3712). IEEE.

[14] Ioffe, S. and Szegedy, C., 2015. Batch normalization: Accelerating deep network training by reducing internal covariate shift. arXiv preprint arXiv:1502.03167.

[15] Santurkar, S., Tsipras, D., Ilyas, A. and Madry, A., 2018. How does batch normalization help optimization?. In Advances in Neural Information Processing Systems (pp. 2483-2493).

[16] Bjorck, N., Gomes, C.P., Selman, B. and Weinberger, K.Q., 2018. Understanding batch normalization. In Advances in Neural Information Processing Systems (pp. 7694-7705).

[17] Mishkin, D. and Matas, J., 2015. All you need is a good init. arXiv preprint arXiv:1511.06422.

[18] Lei Ba, J., Kiros, J.R. and Hinton, G.E., 2016. Layer normalization. arXiv preprint arXiv:1607.06450.

[19] Ulyanov, D., Vedaldi, A. and Lempitsky, V., 2016. Instance normalization: The missing ingredient for fast stylization. arXiv preprint arXiv:1607.08022.

[20] Wu, Y. and He, K., 2018. Group normalization. In Proceedings of the European Conference on Computer Vision (ECCV) (pp. 3-19).

[21] Singh, S. and Krishnan, S., 2019. Filter Response Normalization Layer: Eliminating Batch Dependence in the Training of Deep Neural Networks. arXiv preprint arXiv:1911.09737.

[22] Wang, Y., Wu, X., Chang, Y., Zhang, S., Zhou, Q. and Yan, J., 2018, February. Batch normalization: Is learning an adaptive gain and bias necessary?. In Proceedings of the 2018 10th International Conference on Machine Learning and Computing (pp. 36-40).

[23] Frankle, J., Schwab, D.J. and Morcos, A.S., 2020. Training BatchNorm and Only BatchNorm: On the Expressive Power of Random Features in CNNs. arXiv preprint arXiv:2003.00152.

[24] Goodfellow, I., Bengio, Y., and Courville, A. (2016). Deep learning. MIT press.

[25] Zhang, H., Cisse, M., Dauphin, Y. N., and Lopez-Paz, D. (2017). mixup: Beyond empirical risk minimization. arXiv preprint arXiv:1710.09412.

[26] Krogh, A., and Hertz, J. A. (1992). A simple weight decay can improve generalization. In Advances in neural information processing systems (pp. 950-957).

[27] Selvaraju, R. R., Cogswell, M., Das, A., Vedantam, R., Parikh, D., and Batra, D. (2017). Grad-cam: Visual explanations from deep networks via gradient-based localization. In Proceedings of the IEEE international conference on computer vision (pp. 618-626).


[29] Müller, R., Kornblith, S., and Hinton, G. E. (2019). When does label smoothing help?. In Advances in Neural Information Processing Systems (pp. 4696-4705).

[30] Guo, C., Pleiss, G., Sun, Y., and Weinberger, K. Q. (2017, August). On calibration of modern neural networks. In Proceedings of the 34th International Conference on Machine Learning-Volume 70 (pp. 1321-1330). JMLR. org.


[28] Gal, Y., and Ghahramani, Z. (2016, June). Dropout as a bayesian approximation: Representing model uncertainty in deep learning. In international conference on machine learning (pp. 1050-1059).

[31] Brier, G. W. (1950). Verification of forecasts expressed in terms of probability. Monthly weather review, 78(1), 1-3.

==> deleted/chart-details.tex <==
\begin{SCfigure}
%\begin{figure}[h]
\includegraphics[width=0.5\textwidth, scale=0.6]{figures/100epoch.png}
\caption{Test accuracy vs epoch numbers w.r.t. Batch Norm True and False. As it is the case with test F1 score vs batch numbers, the test accuracy with final Batch Norm layer jumps to above 94\% just after 6th epoch and steadily decreases to 78\% after 100th epoch. But the test accuracy without final Batch Norm layer starts with 67\% and oscillates in a large range between 61\% to 88\% (e57) and then ends at 79\% after 100th epoch.
}
\label{fig:100epoch}
%\end{figure}
\end{SCfigure}



\begin{itemize}
\vspace{-0.2cm}\item Adding a final Batch Norm layer just before the output layer 
\vspace{-0.2cm}\item Freezing or unfreezing (learnable vs pre-trained weights) the previous Batch Norm layers in ResNet34
\vspace{-0.2cm}\item Weighted Cross-Entropy Loss [24] according to class imbalance
\vspace{-0.2cm}\item Data augmentation
\vspace{-0.2cm}\item Mixup [25]
\vspace{-0.2cm}\item Weight decay [26]
\end{itemize}

==> deleted/class_activations_figure.tex <==

In order to see what the model actually sees during training, we visualized the activations on the final CNN layer. Usually, the heatmaps generated are not class-discriminative, i.e.~they only correspond to activations generated in the forward pass through the network. Selvaraju et al.~\cite{selvaraju2017grad} devised a way to visualize which parts of an input image result in the prediction of a specific class. In this study, we used this approach to generate class-discriminative heatmaps. Looking at Figure~\ref{fig:activations}, we see that the model without final BN layer looks at the wrong part of the picture while predicting. The highlighted parts (heatmap) basically tell us which parts of an image induced the wrong classification. In this example, the model made the wrong prediction because of the highlighted part.

%\begin{figure}[h]
%\includegraphics[width=\textwidth]{figures/activations.png}
%\caption{Class discriminative activations while predicting}
%\label{fig:activations}
%\end{figure}

\begin{figure}[h]
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=1.0\linewidth]{figures/activations_bn_false.png}
\subcaptionbox{\textbf{Final BN = False.} Wrong prediction. The activations for unhealthy class is glowing on the wrong pixels and it is predicted as healthy as the glowing parts look healthy (clean). The probability of being unhealthy is 36\% (we some some minor activations close to defected parts). There is no activation happening for healthy class.\label{fig:actbnfalse}}[.9\linewidth]

\end{subfigure}
\begin{subfigure}{0.5\textwidth}
\includegraphics[width=1.0\linewidth]{figures/activations_bn_true.png}
\subcaptionbox{\textbf{Final BN = True.} Correct prediction by a close margin ( 51\%). The activations for unhealthy class is glowing on the right pixels and it is predicted as unhealthy as the glowing parts look unhealthy (defects). The activations for healthy class is also glowing on the right pixels but still shows some defects.\label{fig:actbntrue}}[.9\linewidth]

\end{subfigure}
\caption{Class-discriminate activations for an unhealthy Apple leaf during prediction.}
\label{fig:activations}
\end{figure}


==> deleted/dual_chart_losses.tex <==
\begin{figure}[h]
\includegraphics[width=\textwidth]{figures/vgg_bn_metrics_v5.png}
\caption{\vk {I duplicated this chart to let you see another version with WL. We will remove one} Average (10 runs) loss charts for Apple plant without (left) and with (right) final BN layer in VGG19 architecture. After adding the final BN layer, the test F1 score is increased from 0.2942 to 0.9562 for unhealthy (minority) class while the train and validation losses level off around 0.5 before the model starts overfitting. We also observe that the standard deviation between runs are much lower and training becomes smoother in the later case.}
\label{fig:apple_loss}
\end{figure}

==> deleted/low_probabilities_table.tex <==


\begin{table}[htbp]
\caption{Softmax output values (representing class probabilities) for five images of unhealthy $\mbox{class}=1$ plants. Left column: Without final BN layer, softmax output value for $\mbox{class}=0$ (healthy, wrong classification). Right column: With final BN layer, softmax output value for $\mbox{class}=1$ (unhealthy, correct classification)."}

\label{confident_wrongs}
\begin{tabular}{lllll}
\multicolumn{1}{l}{bn\_false\_class\_0\_prob} &
  \multicolumn{1}{l}{bn\_false\_class\_1\_prob} &
  \multicolumn{1}{l}{bn\_true\_class\_0\_prob} &
  \multicolumn{1}{l}{bn\_true\_class\_1\_prob} &
  \multicolumn{1}{l}{ground\_truth} \\\hline
0.8917 & 0.1082 & 0.4891  & 0.5108 & 1 \\
0.8535 & 0.1464 & 0.3630 & 0.6369 & 1 \\
0.8000  & 0.1999 & 0.3917 & 0.6082  & 1 \\
0.7274  & 0.2725  & 0.3133  & 0.6866 & 1 \\
0.6661 & 0.3338   & 0.2967 & 0.7032  & 1 \\ \hline
\end{tabular}
\end{table}


==> deleted/old_abstract.tex <==
In real world settings, especially in agriculture and healthcare,  anomalies are rare and collecting new samples is usually expensive and time consuming while it is nearly impossible to correctly identify them. In this kind of highly imbalanced classification problem,  deep learning (DL) favors majority classes over minority classes.  In our experiments, we artificially sampled a highly imbalanced data set (99\% vs 1\%) for certain plant types  out of PlantVillage data set to develop methods in classifying the rare diseases through transfer learning. We randomly picked 1000 healthy and 10 unhealthy samples from certain plant types for a training set, fine tuned using ResNet34 and VGG19 CNN architectures,  and then tested the model performance on an equal number of healthy and unhealthy images (150 vs 150) in a test set.  We observed that the initial F1 test score jumped from 0.25 to 0.96 for the minority class when we added a final Batch Normalization (BN) layer just before the output layer. That is, we managed to correctly predict 143 of 150 unhealthy images spanning over multiple anomalies that may not exist in the training or validation set. We illustrate that putting an additional BN layer before the output layer in modern CNN architectures has a considerable impact in terms of minimizing the training time and test error for minority classes in a highly imbalanced data set.
We also illustrate that when the final BN is used, trying to minimize validation and train losses may not be an optimal way for getting a high F1 test score for minority classes in anomaly detection problems and using the final BN layer has a calibration effect. That is, the network might perform better even if it is not ‘confident’ enough while making a prediction; leading to another discussion about why softmax output is not a good uncertainty measure for DL models.


==> deleted/run_onservation_text.tex <==

\comment{
It was using Apple plants, we obtain 0.44 F1 test score on the minority class (unhealthy) and 0.73 on the majority class. When training this model for 10 epochs using Apple plant, we obtained an F1 test score of 0.93 both on minority and majority classes. That is, just by adding a final BN layer test F1 score for the minority class is increased from 0.44 to 0.93 in ResNet34. We then tested this approach in VGG19 and test F1 score for the minority class is increased from 0.25 to 0.96. For detailed metrics and charts, see Figure~\ref{fig:apple_loss} and Table~\ref{tab:three_plants}. We also run the same tests with Pepper and Tomato plants in ResNet34 and observed similar performance improvements.}

\comment {\vk {when I first wrote this paragraph, we didn't have 10-run averages. So, these numbers belong to single runs and do not match with the numbers in table 1 or figure 2. So, to make this paragraph and table1 compatible with the figure 2, I will rerun the tests in VGG19 for 3 plants for 10 runs and update table 1 accordingly. And this paragraph will only mention some key metrics from both table 1 and figure 2. Moreover, we don't even need to mention accuracy in test metrics as it is equal to average of F1 scores in both classess in perfectly balanced datasets (150 vs 150) (i.e. (0.9481 + 0.9518)/2=0.95).
and after dropping accuracy column, we can even make this table transposed and with vs without BN would be first column and we would save some space}}


==> deleted/skin_cancer.tex <==


\subsection {Experiments with ISIC Skin Cancer Dataset}

In order to see the effects of adding the final BN layer in another image datasets, we also run some tests on ISIC Skin Cancer Dataset [12] and tried to classify benign and malignant lesion images using the same class imbalance settings. 

Without using final BN layer, we trained for 10 epochs and the model started to overfit at 7th epoch. Then  we retrained and stopped at 7th epoch. For minority class, the validation F1 score was 0.0, and test F1 score was 0.06.

By adding the final BN layer, we could be able to train for 10 epochs, and for the minority class, the validation F1 score was 0.15, and test F1 score was 0.37. That is, we were able to improve the model accuracy by 31\% increase (from 0.06 to 0.37) in minority class.

==> tables/PlantVillage_SOTA_metrics.tex <==
The classification report for that model can be found in Table~\ref{clf_report}.

\begin{table}[htbp]
\caption{Resnet34 classification report on PlantVillage}
\label{clf_report}
\begin{tabular}{rrrrr}
epoch & train\_loss & valid\_loss & accuracy & error\_rate \\
\toprule
0 & 0.330473 & 0.144808 & 0.952563 & 0.047437 \\
1 & 0.174927 & 0.073233 & 0.975827 & 0.024173 \\
2 & 0.106667 & 0.042294 & 0.985914 & 0.014086 \\
3 & 0.074274 & 0.031119 & 0.990367 & 0.009633 \\
4 & 0.049989 & 0.027862 & 0.990731 & 0.009269 \\
5 & 0.047698 & 0.026165 & 0.992003 & 0.007997 \\
6 & 0.029981 & 0.019031 & 0.993548 & 0.006452 \\
7 & 0.009868 & 0.008603 & 0.997365 & 0.002635 \\
8 & 0.005390 & 0.007651 & 0.997546 & 0.002454 \\
9 & 0.006720 & 0.007472 & 0.997819 & 0.002181\\
\bottomrule
\end{tabular}
\end{table}

==> tables/plant_village_stats.tex <==
The number of samples in each plant type can be found at Table~\ref{plant_dataset}.

\begin{table}[htbp]
\caption{PlantVillage dataset}
\label{plant_dataset}
\begin{tabular}{lrrrr}
 & \multicolumn{1}{l}{Train set} & \multicolumn{1}{l}{}          & \multicolumn{1}{l}{Validation set} & \multicolumn{1}{l}{}          \\
 & \multicolumn{1}{l}{healthy}   & \multicolumn{1}{l}{unhealthy} & \multicolumn{1}{l}{healthy}        & \multicolumn{1}{l}{unhealthy} \\
\toprule
Potato     & 121  & 1600  & 31   & 400  \\
Peach      & 288  & 1838  & 72   & 459  \\
Cherry     & 684  & 842   & 170  & 210  \\
Grape      & 339  & 2912  & 84   & 727  \\
Tomato     & 1272 & 13132 & 318  & 3284 \\
Pepper     & 1181 & 797   & 295  & 200  \\
Corn       & 16   & 2005  & 5    & 503  \\
Orange     & 0    & 4405  & 0    & 1102 \\
Blueberry  & 1202 & 0     & 300  & 0    \\
Apple      & 1316 & 1220  & 329  & 306  \\
Squash     & 0    & 1448  & 0    & 365  \\
Soybean    & 4072 & 0     & 1018 & 0    \\
Raspberry  & 297  & 0     & 74   & 0    \\
Strawberry & 364  & 886   & 92   & 222 \\
\bottomrule
\end{tabular}
\end{table}

\begin{table}[]
\caption{}
\label{tab:my-table}
\begin{tabular}{|l|c|l|c|l|c|}
\hline
 & \multicolumn{1}{l|}{} & \multicolumn{1}{c|}{with final BN layer} &               & \multicolumn{1}{c|}{without final BN layer} &               \\ \hline
 & class                 & \multicolumn{1}{c|}{test F1}             & test accuracy & \multicolumn{1}{c|}{test F1}                & test accuracy \\ \hline
Apple  & Unhealthy & 0.9481 & 0.9500 & 0.4211 & 0.6333 \\ \hline
       & Healthy   & 0.9518 &        & 0.7317 &        \\ \hline
Pepper & Unhealthy & 0.9439 & 0.9433 & 0.6301 & 0.7300 \\ \hline
       & Healthy   & 0.9428 &        & 0.7874 &        \\ \hline
Tomato & Unhealthy & 0.9833 & 0.9833 & 0.6301 & 0.7300 \\ \hline
       & Healthy   & 0.9834 &        & 0.7874 &        \\ \hline
\end{tabular}
\end{table}
